GuardianAgentFlow: Multi-Agent Coordination for Web Privacy Protection

Web agents need to use private context without unnecessarily disclosing it. Effective protection must distinguish between requests that may be sent after sanitization and those that must be withheld, while preserving the information needed for authorized tasks. We present GuardianAgentFlow, a multi-agent framework that mediates outgoing Web requests through an explicit release contract. A dedicated restriction check grounds permission in the user's instruction; a shared protection scope aligns rewriting with disclosure checking; and candidate-grounded feedback guides revision before transmission. Experiments on Web requests with human-reviewed intent labels show improved request-contract success, while controlled comparisons and role ablations identify the contributions of restriction handling, policy evidence, and candidate checking. Evaluations of action proposals from PrivacyLens and AgentDAM demonstrate complementary protection when mediation is composed with privacy-aware agents. Experiments with smaller mediation models show that the coordination benefit persists with reduced model capacity. Dedicated-server measurements show lower mediation latency than full-policy reasoning, while real-site browser tests quantify integration overhead.

==> sections/limitations.tex <==
\section{System Implications}
\label{sec:limitations}
\label{sec:eval-interpretation}
The results favor a division of responsibility organized around the outgoing action. Permission analysis determines whether transmission is authorized, the shared scope specifies what may survive, and candidate verification checks the actual replacement. A role can therefore change its internal reasoning without silently changing the next role's objective. The contract exposes the relevant intermediate state for both diagnosis and intervention: a wrong permission branch calls for instruction analysis, an overly broad scope calls for task-context reasoning, and a residual disclosure calls for candidate repair.

This organization also explains the deployment tradeoff. A one-call mediator offers a short execution path; \sys{} spends additional computation where explicit restrictions and revisions improve completion. Against full-policy reasoning, scoped evidence and conditional rewriting improve both request success and measured latency. The same release interface accommodates an upstream privacy-aware agent, allowing context minimization and outgoing-content checking to contribute at separate stages. Together, the ablations, layering experiments, and timing measurements support modular coordination as the system contribution.

